Process Discovery Using Graph Neural Networks

Automatically discovering a process model from an event log is the prime problem in process mining. This task is so far approached as an unsupervised learning problem through graph synthesis algorithms. Algorithmic design decisions and heuristics allow for efficiently finding models in a reduced search space. However, design decisions and heuristics are derived from assumptions about how a given behavioral description - an event log - translates into a process model and were not learned from actual models which introduce biases in the solutions. In this paper, we explore the problem of supervised learning of a process discovery technique D. We introduce a technique for training an ML-based model D using graph convolutional neural networks; D translates a given input event log into a sound Petri net. We show that training D on synthetically generated pairs of input logs and output models allows D to translate previously unseen synthetic and several real-life event logs into sound, arbitrarily structured models of comparable accuracy and simplicity as existing state of the art techniques for discovering imperative process models. We analyze the limitations of the proposed technique and outline alleys for future work.

==> 2_background.tex <==
We write $A$ for the (finite) set of \emph{activity names} extended with $>\in A$ and $| \in A$ for artificial start and end. A \emph{log} $L$ (over $A$) is a finite multiset of traces where a \emph{trace} is a finite sequence $\sigma = \langle >, a_1,\ldots,a_n,| \rangle \in A^*$. Each occurrence of an activity $a_i \in \sigma$ is called an \emph{event}.

We recall notations for Petri nets with $\tau$-transitions and refer to~\cite{DBLP:journals/cj/VerbeekBA01} for definitions. A Petri net $N = (P,T_A \cup T_\tau,F)$ has places $P$, transitions $T = T_A \cup T_\tau$ where $T_A$ and $T_\tau$ are \emph{visible} and \emph{invisible} transitions (i.e., do not occur in firing sequences of $N$), respectively, and arcs $F$. In a \emph{workflow net} $N$, every node of $N$ is on a path (along $F$) from the unique source place $i \in P$ (no incoming arcs) to the unique sink place $o$ (no outgoing arcs).

%\begin{definition}{(Activity, Trace, Event log)}\label{def:event_log}
%Let $A$ be the set of all possible activities, let $>\in A$ and $| \in A$ be artificial start and end activities. A trace is a sequence containing $>$ as the first element, $|$ as the last element and in-between elements of $A\setminus\{>,|\}$. Let $\mathcal{T}$ be the set of all such traces. A log $L \subseteq \mathbb{M}(\mathcal{T})$ is a multiset of traces. The set of distinct traces is both denoted as trace variants and the log's behavior $\mathcal{B}(L)$.
%\end{definition}

%\begin{definition}{(Alpha relations)}\label{def:alpha_relations}
%Let $L$ be a log and $\Sigma(L)$ the distinct events therein. Let $a, b \in \Sigma(L)$:
%\begin{itemize}[label=\raisebox{0.25ex}{\tiny$\bullet$}]
%    \item directly follows relation: $a >_L b \iff \exists T = \left< t_1t_2t_3\dots t_{n} \right> \wedge 1 \leq i \leq n-1: T \in L, t_i = a, t_{i+1} = b$;
%    \item eventually follows relation: $a >^f_L b \iff \exists T = \left< t_1t_2t_3\dots t_{n} \right> \wedge 1 \leq i \leq n-1: T \in L, t_i = a, t_{i+f} = b$;
%    \item causal relation: $a \rightarrow_L b \iff a >_L b \wedge b \ngeq_L a$;
%    \item no relation: $a \#_L b \iff a \ngeq_L b \wedge b \ngeq_L a$;
%    \item parallel relation: $a \|_L b \iff a >_L b \wedge b >_L a$;
%    \item cycle relation: $\circlearrowleft_La \iff \exists T = \left< t_1t_2t_3\dots t_{n} \right> \wedge 1 \leq i, j \leq n-1, i < j: T \in L, t_i = a, t_j = a$.
%\end{itemize}
%\end{definition}


